Exorcising ''Wraith'': Protecting LiDAR-based Object Detector in Automated Driving System from Appearing Attacks

Automated driving systems rely on 3D object detectors to recognize possible obstacles from LiDAR point clouds. However, recent works show the adversary can forge non-existent cars in the prediction results with a few fake points (i.e., appearing attack). By removing statistical outliers, existing defenses are however designed for specific attacks or biased by predefined heuristic rules. Towards more comprehensive mitigation, we first systematically inspect the mechanism of recent appearing attacks: Their common weaknesses are observed in crafting fake obstacles which (i) have obvious differences in the local parts compared with real obstacles and (ii) violate the physical relation between depth and point density. In this paper, we propose a novel plug-and-play defensive module which works by side of a trained LiDAR-based object detector to eliminate forged obstacles where a major proportion of local parts have low objectness, i.e., to what degree it belongs to a real object. At the core of our module is a local objectness predictor, which explicitly incorporates the depth information to model the relation between depth and point density, and predicts each local part of an obstacle with an objectness score. Extensive experiments show, our proposed defense eliminates at least 70% cars forged by three known appearing attacks in most cases, while, for the best previous defense, less than 30% forged cars are eliminated. Meanwhile, under the same circumstance, our defense incurs less overhead for AP/precision on cars compared with existing defenses. Furthermore, We validate the effectiveness of our proposed defense on simulation-based closed-loop control driving tests in the open-source system of Baidu's Apollo.

==> mail2.tex <==
Dear Shepherd,

Thank you very much for your and other reviewers' suggestions on our recent submission!

First of all, we are very sorry for our carelessness and all the typos and grammar errors appeared in the system integration part of the Section 5.4 and the Appendix H. We have carefully revised these parts again, and we promise that there will be no more typos or grammar errors in these parts.

Besides, we are sorry that we don't clearly describe the details of our system integration experiments in our submission, such as how we perform these experiments, how we calculate the crash rate and why we perform the system-level experiments in such way. Specifically, to perform these experiments, we first select 5 different fake PCs which are located in front of the self-driving vehicle and can successfully forged the perception module of Apollo or those 3D object detectors for at least 1 frame in the previous experiments. Meanwhile, we use Apollo to record 3 traces of the self-driving vehicle moving in different maps under the manual control. Then, we inject the selected fake PCs into all the frames of these traces to generate 15 different poisoned traces. 

During the experiments, we run Apollo 6.0.0 system with and without LOP in the poisoned traces and visualize the future routes generated by the planning module of Apollo, which are shown as the green rectangles in front of the self-driving vehicle. We also assume that there is a car moving behind the self-driving vehicle at a constant speed as the potential crash target. The generated future routes represent the moving trajectories of the self-driving vehicle under the control of Apollo, which can help us determine whether the self-driving vehicle will suddenly brake in the corresponding circumstances, and indirectly indicate a potential crash.

As shown in the part (a) of Fig.13, the generated future route is extended to the crossroads, which means the self-driving vehicle will moving normally and stop at a red light under the instructions of the Apollo with our LOP. Therefore, we consider this situation as the ``no accident''. Meanwhile, as shown in the part (b) of Fig.13, the generated future route disappears for a while, which means the self-driving vehicle will falsely brake in the middle of the road, and crash with the imaginary car moving behind it as we mentioned above. Therefore, we consider this situation as the ``car crash''. We calculates the proportion of the ``car crash'' in the 15 poisoned traces as the crash rate, and report it in the Section 5.4.

The main reason why we calculate the crash rate in such a complex way is that we are facing some problems in bridging the LGSVL simulator and the Apollo, which are difficult to solve in a short time. Specifically, the regular bridging methods will directly send the ground-truth detection results of objects nearby the self-driving vehicle to Apollo. It means that it is impossible for appearing attacks to successfully forge objects, since the Apollo will bypass the perception module during the simulation.

Moreover, we think the details of these experiments are a little bit redundancy for our paper, so we incorporate the explanation above in the Appendix H of our submission instead. 

We provide the draft and the diff file which highlights the difference between this submission and the previous submission in the attachments. If you have any further suggestions on our system-level experiments or other parts of our work, please let us know. Thank you again for your valuable help and constructive suggestions:)  

Best Regards!

==> table/attack_comp_table_backup.tex <==
\begin{table}[t]
  \centering
  \vspace{-0.2in}
  \caption{The AP on cars of 3D object detectors with and without LOP or other defense methods under attacks.
%   "PointNet" and "DGCNN" refers to the model structure of LOP, \louis{with a boundary value $B$} used to distinguish real objects and fake objects as the description in Section \ref{sec:method:voting}."LPD" and "FSD" are two different strategies for CARLO to calculate the anomalous ratio, and $M,\ k,\ r$ are the hyper-parameters of other defenses, which are all described in Section \ref{sec:Limitation}.
  }
\scalebox{0.5}{
    \begin{tabular}{lccccccc}
    \toprule
          & \multicolumn{2}{c}{PointPillars} & \multicolumn{3}{c}{PointRCNN} & \multicolumn{2}{c}{PV-RCNN} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-8}          & Physical & Baseline  & Physical & Baseline  & Roadside & Physical & Baseline \\
    \midrule
    w/o. defense  & 70.06\% & 68.57\% & 67.92\% & 65.95\% & 61.59\% & 70.11\% & 66.39\% \\
    SRS (M=500) & 70.12\% & 68.55\% & 69.42\% & 65.44\% & 62.48\% & 70.14\% & 66.27\% \\
    \midrule
    SOR (k=2) & 70.43\% & 68.84\% & 72.56\% & 65.41\% & 60.84\% & 71.43\% & 64.80\% \\
    SOR (k=10) & 70.01\% & 68.06\% & 72.63\% & 65.26\% & 60.53\% & 71.28\% & 64.09\% \\
    \midrule
    CARLO(FSD, R=0.6) & 65.94\% & 63.49\% & 67.16\% & 63.53\% & 60.16\% & 67.99\% & 63.27\% \\
    CARLO(FSD, R=0.7) & 69.60\% & 67.96\% & 68.41\% & 65.29\% & 60.71\% & 70.10\% & 66.07\% \\
    CARLO(FSD, R=0.8) & 69.64\% & 67.96\% & 68.15\% & 65.22\% & 60.69\% & 70.15\% & 65.84\% \\
    CARLO(LPD, R=0.6) & 67.79\% & 64.37\% & 68.98\% & 65.27\% & 60.53\% & 69.23\% & 64.46\% \\
    CARLO(LPD, R=0.7) & 69.57\% & 67.99\% & 69.22\% & 65.97\% & 61.41\% & 70.26\% & 65.71\% \\
    CARLO(LPD, R=0.8) & 69.82\% & 68.49\% & 69.15\% & 66.04\% & 61.65\% & 70.35\% & 66.11\% \\
    \midrule
    Shadow-Catcher(Threshold=0.2) & 47.72\% & 57.81\% & / & / & / & / & / \\
    Shadow-Catcher(Threshold=0.4) & 75.46\% & 75.03\% & / & / & / & / & / \\
    Shadow-Catcher(Threshold=0.6) & \textbf{77.05\%} & \textbf{75.95\%} & / & / & / & / & / \\
    \midrule
    Ours(PointNet, B=0.5) & 70.92\% & 69.50\% & 73.32\% & 71.87\% & 70.82\% & 71.47\% & 69.25\% \\
    Ours(PointNet, B=0.6) & 70.97\% & 69.63\% & \textbf{73.77\%} & 72.30\% & 71.41\% & 71.86\% & 69.19\% \\
    Ours(DGCNN, B=0.5) & 71.11\% & 69.72\% & 73.07\% & 72.29\% & 71.99\% & \textbf{71.87\%} & \textbf{69.88\%} \\
    Ours(DGCNN, B=0.6) & 70.39\% & 68.61\% & 73.74\% & \textbf{73.42\%} & \textbf{72.84\%} & 71.51\% & 68.30\% \\
    \bottomrule
    \end{tabular}%
}
%   \vspace{-0.1in}
  \label{tab:comp_map_atk}%
\end{table}%

==> table/normal_comp_table_backup.tex <==
\begin{table}[ht]
  \centering
  \vspace{-0.2in}
  \caption{The AP and precision of 3D object detectors on cars with and without LOP or other defense methods on clean samples.}
\scalebox{0.55}{
    \begin{tabular}{lcccccc}
    \toprule
          & \multicolumn{2}{c}{PointPillars} & \multicolumn{2}{c}{PointRCNN} & \multicolumn{2}{c}{PV-RCNN} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}          & AP    & Precision & AP    & Precision & AP    & Precision \\
    \midrule
    w/o. defense  & 72.34\% & 78.99\% & 75.13\% & 75.04\% & 73.32\% & 73.12\% \\
    SRS (M=500) & 72.33\% & 79.14\% & 75.52\% & 74.75\% & 73.48\% & 73.23\% \\
    \midrule
    SOR (k=2) & 71.20\% & 78.91\% & 74.46\% & 74.49\% & 72.52\% & 72.92\% \\
    SOR (k=10) & 70.58\% & 78.86\% & 74.04\% & 73.88\% &72.22\% & 72.94\% \\
    \midrule
    CARLO(LPD, R=0.6) & 67.92\% & 75.06\% & 73.49\% & 73.10\% & 71.43\% & 70.08\% \\
    CARLO(LPD, R=0.7) & 72.03\% & 77.81\% & 74.63\% & 74.35\% & 73.21\% & 72.22\% \\
    CARLO(LPD, R=0.8) & 71.95\% & 78.00\% & 74.53\% & 74.32\% & 73.20\% & 72.41\% \\
    CARLO(FSD, R=0.6) & 69.80\% & 75.77\% & 74.17\% & 73.07\% & 72.00\% & 69.93\% \\
    CARLO(FSD, R=0.7) & 71.58\% & 77.56\% & 74.79\% & 74.38\% & 72.94\% & 71.66\% \\
    CARLO(FSD, R=0.8) & 72.02\% & 78.31\% & 74.89\% & 74.87\% & 73.15\% & 72.37\% \\
    \midrule
    Shadow-Catcher(Threshold=0.2) & 50.58\% & 70.25\% & / & / & / & / \\
    Shadow-Catcher(Threshold=0.4) & 77.41\% & 77.31\% & / & / & / & / \\
    Shadow-Catcher(Threshold=0.6) & \textbf{79.47\%} & 76.91\% & / & / & / & / \\
    \midrule
    Ours(PointNet, B=0.5) & 72.86\% & 81.77\% & 76.49\% & 79.29\% & 73.65\% & 77.85\%  \\
    Ours(PointNet, B=0.6) & 72.88\% & 82.38\% & 76.37\% & 80.03\% & 73.80\% & 78.53\% \\
    Ours(DGCNN, B=0.5) & 73.63\% & 83.04\% & 76.77\% & 80.75\% & \textbf{74.50\%} & 79.61\% \\
    Ours(DGCNN, B=0.6) & 72.73\% & \textbf{83.90\%} & \textbf{76.84\%} & \textbf{81.52\%} & 73.86\% & \textbf{80.34\%} \\
    \bottomrule
    \end{tabular}%
}
%   \vspace{-0.1in}
  \label{tab:comp_normal_pre}%
\end{table}%

==> tex/ODsetting.tex <==
\section{Experiment Settings of 3D Object Detectors} \label{app:ODsetting}

==> tex/ablation.tex <==
\section{Related Work} \label{sec:relatedWork}

==> tex/alg/detection.tex <==

\begin{algorithm}[ht]
  \caption{Fake Object Elimination}
  \label{alg:detecting}
\begin{algorithmic}[1]
  \STATE {\bfseries Input:} Input PC $X_t$, input space $D$, threshold $\beta$.
  \STATE {\bfseries Input:} Local objectness predictor $O$, boundary value $B$.
  \STATE {\bfseries Input:} Detector's original prediction $Preds$.
  \STATE {\bfseries Output:} Detector's final prediction $\overline{Preds}$.
  \STATE Split $D$ into equal-sized pillars: $Pillars = \text{split}(D)$.
  \FOR{Pillar $p_j\in Pillars$}
  \FOR{Point $x_i\in X_t$}
  \STATE Initialize: $pc_j=\emptyset$.
  \IF{$x_i$ {\bfseries inside} $p_j$}
  \STATE Generate a $7$-dim feature vector $x_i'$ for $x_i$.
  \STATE $pc_j=pc_j\bigcup x_i'$.
  \ENDIF
  \ENDFOR
  \STATE Calculate the objectness score: $\widehat{obj_j}=O(pc_j)$.
  \ENDFOR
  \STATE Initialize: $\overline{Preds}=\emptyset$.
  \FOR{$pred_k\in Preds$}
  \STATE Initialize: $cnt_k = 0, sum_k = 0$.
  \FOR{Pillar $p_j\in Pillars$}
  \IF{$IoU_{2D}(pred_k,p_j)>\beta$}
  \STATE $sum_k+=\widehat{obj_j}$
  \STATE $cnt_k+=1$
  \ENDIF
  \ENDFOR
  \IF{$sum_k/ cnt_k>B$}
  \STATE $\overline{Preds}=\overline{Preds}\bigcup pred_k$.
  \ENDIF
  \ENDFOR
  \RETURN $\overline{Preds}$
\end{algorithmic}
\end{algorithm}

==> tex/app_FP.tex <==
\section{A Case Study of the False Positives}
\label{appendix:FP}
Specifically, we investigate the origin of the false positives with the three factors: the size, the depth and the density of the detected objects. In our analysis, we randomly select $1000$ sample frames of point clouds from the validation set of KITTI, and calculate the three factors above for the contained objects.

%%%%%%%% BEGIN FP
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/FP_analysis.png}
    \caption{The Visualization of false positive detected by our LOP, where the solid boxes refer to the remained real vehicles after LOP's detection, and dashed boxes refer to the real vehicles erased by LOP.}
    \label{fig:FP_analysis}
\end{figure}
%%%%%%%% END FP

Indeed, the distribution of the false positives and the true positives are similar to one another in terms of the size and the density, while non-trivial differences exist in their depth. Specifically, false negatives are relatively more likely to exist when the depth is larger: the ratio between the false positive with depth less than $10$m and those with depth more than $10$m is $1:7.37$, while the ratio between the false positive with depth less than $20$m and those with depth more than $20$m is $1:5.05$. Furthermore, the number of false positive with depth less than $10$m is only $1.60\%$ of the total real vehicles, and the number of false positive with depth less than $10$m is only $2.21\%$ of the total real vehicles. The results indicate that our LOP may not recognize the forged obstacles well in some cases due to its imprecision on distant vehicles. 

For better intuition, we visualize one sample scenario in Fig.\ref{fig:FP_analysis}. As we can see, compared with the false positives (marked in dotted lines), the true positives usually have a lower depth and its point density were unevenly distributed and dense in some specific parts. Therefore, the true positives usually have less pillars which however contain sufficient points for LOP to analyze. Therefore, they were easier to be detected with the sufficient information contained in the dense pillars. In contrast, the pillars in false positives are almost evenly sparse and hence would increase the uncertainty of our LOP's prediction. The visualization explains why LOP is limited in recognizing some distant crafted objects. 

Finally, due to the existence of the MOT module, which tracks the detected objects and supply the trajectories of nearby objects for further route planning, the self-driving system will keep refreshing the driving plan and correct the mis-prediction of distant objects when it comes nearby. Moreover, MOT would prevent the self-driving system from ignoring a distant object only if LOP misses a distant object in several consecutive frames, the possibility of which is less than $1\%$ according to our calculation. Therefore, the negative influence of LOP on the normal performance of a detector can be further limited.

==> tex/app_ablation_backup.tex <==
\section{Hyper-parameter Sensitive Experiments on PointPillars and PV-RCNN}
\label{appendix:ablation}

% Fig.\ref{fig:ablation_PPPV_normal} 
Table \ref{tab:ablation_PP_normal} and \ref{tab:ablation_PV_normal}
show
the AP and precision of PointPillars and PV-RCNN when deploying the LOP with different hyper-parameters in the normal circumstances, and Fig.\ref{fig:ablation_PPPV_atk} shows the ASR of different attacks and the precision of PointPillars and PV-RCNN when deploying the LOP with different hyper-parameters under attacks.
% the detectors' AP and precision of LOP on PointPillars and PV-RCNN in the normal circumstances, and Fig.\ref{fig:ablation_PPPV_atk} shows the defense effectiveness and the detectors' precision of LOP on PointPillars and PV-RCNN under attack.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figs/ablation_PPPV_normal.png}
%     \caption{The results of hyper-parameter sensitive experiment on PointPillars and PV-RCNN in normal circumstance.}
%     \label{fig:ablation_PPPV_normal}
% \end{figure}

\begin{table}[ht]
  \centering
  % \vspace{-0.2in}
  \caption{The results of hyper-parameter sensitive experiment on PointPillars in the normal circumstances.}
\scalebox{0.7}{
    \begin{tabular}{lcccc}
    \toprule
          & \multicolumn{4}{c}{PointPillars} \\ \cmidrule(lr){2-5}  & AP    & \multicolumn{3}{c}{Precision} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-5}  & Car   & Car   & Pedestrian & Cyclist \\
    \midrule
    w/o. defense  & 72.34\% & 78.99\% & 63.63\% & 59.11\% \\
    \midrule
    Ours(PointNet, B=0.2) & \textbf{73.97\%} & 80.12\% & 63.99\% & 60.09\% \\
    Ours(PointNet, B=0.3) & 72.85\% & 80.46\% & 64.00\% & 59.91\% \\
    Ours(PointNet, B=0.4) & 73.62\% & 81.04\% & \textbf{64.27\%} & 61.34\% \\
    Ours(PointNet, B=0.5) & 72.86\% & 81.77\% & 63.45\% & 61.50\% \\
    Ours(PointNet, B=0.6) & 72.88\% & \textbf{82.38\%} & 63.47\% & \textbf{62.11\%} \\
    \midrule
    Ours(DGCNN, B=0.2) & 73.02\% & 80.88\% & 64.71\% & 60.44\% \\
    Ours(DGCNN, B=0.3) & 73.57\% & 81.41\% & 64.42\% & 60.51\% \\
    Ours(DGCNN, B=0.4) & 72.72\% & 82.20\% & \textbf{64.73\%} & 63.56\% \\
    Ours(DGCNN, B=0.5) & \textbf{73.63\%} & 83.04\% & 64.42\% & 64.89\% \\
    Ours(DGCNN, B=0.6) & 72.73\% & \textbf{83.90\%} & 64.44\% & \textbf{66.45\%} \\
    \bottomrule
    \end{tabular}%
}
  \label{tab:ablation_PP_normal}%
\end{table}%

Similar to the results shown in Section \ref{sec:Experiment:results:ablation}, the effectiveness of our proposed defense on PointPillars and PV-RCNN is also insensitive to different choices of the model structure of LOP, while the value of $B$ will still make influence on the precision of the 3D object detector and the defense effectiveness of LOP under attacks. In short, the LOP with a higher $B$ also performs better on PointPillars and PV-RCNN.

~\\
~\\
% ~\\
% ~\\

\begin{table}[h]
  \centering
  % \vspace{-0.2in}
  \caption{The results of hyper-parameter sensitive experiment on PV-RCNN in the normal circumstances.}
\scalebox{0.7}{
    \begin{tabular}{lcccc}
    \toprule
          & \multicolumn{4}{c}{PV-RCNN} \\ \cmidrule(lr){2-5} & AP    & \multicolumn{3}{c}{Precision} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-5} & Car   & Car   & Pedestrian & Cyclist \\
    \midrule
    w/o. defense & 73.32\% & 73.12\% & 53.34\% & 62.17\% \\
    \midrule
    Ours(PointNet, B=0.2) & \textbf{74.36\%} & 74.83\% & 54.14\% & 62.91\% \\
    Ours(PointNet, B=0.3) & 74.04\% & 75.49\% & \textbf{54.16\%} & 63.30\% \\
    Ours(PointNet, B=0.4) & 74.10\% & 76.50\% & 53.80\% & 63.17\% \\
    Ours(PointNet, B=0.5) & 73.65\% & 77.85\% & 53.13\% & 63.13\% \\
    Ours(PointNet, B=0.6) & 73.80\% & \textbf{78.53\%} & 53.00\% & \textbf{64.99\%} \\
    \midrule
    Ours(DGCNN, B=0.2) & 73.87\% & 76.43\% & \textbf{54.40\%} & 63.94\% \\
    Ours(DGCNN, B=0.3) & 74.34\% & 77.04\% & 51.16\% & 64.35\% \\
    Ours(DGCNN, B=0.4) & 73.99\% & 78.30\% & 53.77\% & 64.93\% \\
    Ours(DGCNN, B=0.5) & \textbf{74.50\%} & 79.61\% & 52.49\% & 66.80\% \\
    Ours(DGCNN, B=0.6) & 73.86\% & \textbf{80.34\%} & 52.43\% & \textbf{68.95\%} \\
    \bottomrule
    \end{tabular}%
}
  \label{tab:ablation_PV_normal}%
\end{table}%

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/ablation_PPPV_attack.png}
    \caption{The results of hyper-parameter sensitive experiment on PointPillars and PV-RCNN under different attacks.
    The precision and ASR metrics are represented in triangles and circles respectively, while the structures of LOP are distinguished in colors.
    The blue horizontal dotted lines in (a), (c) and (b), (d) represent the precision of PointPillars and PV-RCNN on cars respectively in the normal circumstances.
    }
    \label{fig:ablation_PPPV_atk}
\end{figure}

==> tex/app_ablation_backup2.tex <==
\section{Hyperparameter Sensitivity}
\label{appendix:hyper}
\noindent\textbf{Experiment Settings.} To explore the impact of the hyperparameters and the structure of LOP, we implement the LOP with different values of $B$ and different architectures. 
Table \ref{tab:ablation_normal}, Table \ref{tab:ablation_PP_normal} and Table \ref{tab:ablation_PV_normal} report the AP and precision of PointRCNN, PointPillars and PV-RCNN when our defense is deployed with different settings under the normal circumstance. Fig.\ref{fig:ablation_atk} and Fig.\ref{fig:ablation_PPPV_atk} report the defense effectiveness and the precision of PointRCNN, PointPillars and PV-RCNN when our defense is deployed with different settings under attacks.

%%%%%%% BEGIN Ablation
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/PointRCNN_ablation.png}
    \caption{The ASR of different attacks and the precision of PointRCNN when deploying the LOP with different values of $B$ and different model structures on PointRCNN.
    \lyf{The precision and ASR metrics are represented in triangles and circles respectively, while the structures of LOP are distinguished in colors.}
    The blue horizontal dotted lines in (a), (b) and (c) all represent the precision of PointRCNN on cars in the normal circumstances.}
    \label{fig:ablation_atk}
\end{figure*}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/ablation_PPPV_attack.png}
    \caption{The results of hyper-parameter sensitive experiment on PointPillars and PV-RCNN under different attacks.
    The precision and ASR metrics are represented in triangles and circles respectively, while the structures of LOP are distinguished in colors.
    The blue horizontal dotted lines in (a), (c) and (b), (d) represent the precision of PointPillars and PV-RCNN on cars respectively in the normal circumstances.
    }
    \label{fig:ablation_PPPV_atk}
\end{figure}

\begin{table}[ht]
  \centering
  \vspace{-0.2in}
  \caption{The AP and precision of PointRCNN equipped with the LOP with different $B$ and different model structures.}
\scalebox{0.7}{
    \begin{tabular}{lcccc}
    \toprule
          & \multicolumn{4}{c}{PointRCNN} \\
\cmidrule{2-5}          & AP    & \multicolumn{3}{c}{Precision} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-5}          & Car   & Car   & Pedestrian & Cyclist \\
    \midrule
    w/o. defense  & 75.13\% & 75.04\% & 47.08\% & 56.87\% \\
    \midrule
    Ours(PointNet, B=0.2) & 75.96\% & 76.49\% & 50.70\% & 58.66\% \\
    Ours(PointNet, B=0.3) & 76.21\% & 77.15\% & \textbf{50.94\%} & 58.93\% \\
    Ours(PointNet, B=0.4) & \textbf{76.50\%} & 78.05\% & 50.49\% & 61.59\% \\
    Ours(PointNet, B=0.5) & 76.49\% & 79.29\% & 49.63\% & 61.92\% \\
    Ours(PointNet, B=0.6) & 76.37\% & \textbf{80.03\%} & 49.43\% & \textbf{63.87\%} \\
    \midrule
    Ours(DGCNN, B=0.2) & 76.44\% & 77.56\% & 51.04\% & 61.03\% \\
    Ours(DGCNN, B=0.3) & 76.66\% & 78.36\% & \textbf{51.31\%} & 61.72\% \\
    Ours(DGCNN, B=0.4) & 76.58\% & 79.44\% & 51.21\% & 63.74\% \\
    Ours(DGCNN, B=0.5) & 76.77\% & 80.75\% & 49.59\% & 65.14\% \\
    Ours(DGCNN, B=0.6) & \textbf{76.84\%} & \textbf{81.52\%} & 49.42\% & \textbf{67.24\%} \\
    \bottomrule
    \end{tabular}%
}
%   \vspace{-0.1in}
  \label{tab:ablation_normal}%
\end{table}%

\begin{table}[ht]
  \centering
  % \vspace{-0.2in}
  \caption{The results of hyper-parameter sensitive experiment on PointPillars in the normal circumstances.}
\scalebox{0.7}{
    \begin{tabular}{lcccc}
    \toprule
          & \multicolumn{4}{c}{PointPillars} \\ \cmidrule(lr){2-5}  & AP    & \multicolumn{3}{c}{Precision} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-5}  & Car   & Car   & Pedestrian & Cyclist \\
    \midrule
    w/o. defense  & 72.34\% & 78.99\% & 63.63\% & 59.11\% \\
    \midrule
    Ours(PointNet, B=0.2) & \textbf{73.97\%} & 80.12\% & 63.99\% & 60.09\% \\
    Ours(PointNet, B=0.3) & 72.85\% & 80.46\% & 64.00\% & 59.91\% \\
    Ours(PointNet, B=0.4) & 73.62\% & 81.04\% & \textbf{64.27\%} & 61.34\% \\
    Ours(PointNet, B=0.5) & 72.86\% & 81.77\% & 63.45\% & 61.50\% \\
    Ours(PointNet, B=0.6) & 72.88\% & \textbf{82.38\%} & 63.47\% & \textbf{62.11\%} \\
    \midrule
    Ours(DGCNN, B=0.2) & 73.02\% & 80.88\% & 64.71\% & 60.44\% \\
    Ours(DGCNN, B=0.3) & 73.57\% & 81.41\% & 64.42\% & 60.51\% \\
    Ours(DGCNN, B=0.4) & 72.72\% & 82.20\% & \textbf{64.73\%} & 63.56\% \\
    Ours(DGCNN, B=0.5) & \textbf{73.63\%} & 83.04\% & 64.42\% & 64.89\% \\
    Ours(DGCNN, B=0.6) & 72.73\% & \textbf{83.90\%} & 64.44\% & \textbf{66.45\%} \\
    \bottomrule
    \end{tabular}%
}
  \label{tab:ablation_PP_normal}%
\end{table}%

\begin{table}[h]
  \centering
  % \vspace{-0.2in}
  \caption{The results of hyper-parameter sensitive experiment on PV-RCNN in the normal circumstances.}
\scalebox{0.7}{
    \begin{tabular}{lcccc}
    \toprule
          & \multicolumn{4}{c}{PV-RCNN} \\ \cmidrule(lr){2-5} & AP    & \multicolumn{3}{c}{Precision} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-5} & Car   & Car   & Pedestrian & Cyclist \\
    \midrule
    w/o. defense & 73.32\% & 73.12\% & 53.34\% & 62.17\% \\
    \midrule
    Ours(PointNet, B=0.2) & \textbf{74.36\%} & 74.83\% & 54.14\% & 62.91\% \\
    Ours(PointNet, B=0.3) & 74.04\% & 75.49\% & \textbf{54.16\%} & 63.30\% \\
    Ours(PointNet, B=0.4) & 74.10\% & 76.50\% & 53.80\% & 63.17\% \\
    Ours(PointNet, B=0.5) & 73.65\% & 77.85\% & 53.13\% & 63.13\% \\
    Ours(PointNet, B=0.6) & 73.80\% & \textbf{78.53\%} & 53.00\% & \textbf{64.99\%} \\
    \midrule
    Ours(DGCNN, B=0.2) & 73.87\% & 76.43\% & \textbf{54.40\%} & 63.94\% \\
    Ours(DGCNN, B=0.3) & 74.34\% & 77.04\% & 51.16\% & 64.35\% \\
    Ours(DGCNN, B=0.4) & 73.99\% & 78.30\% & 53.77\% & 64.93\% \\
    Ours(DGCNN, B=0.5) & \textbf{74.50\%} & 79.61\% & 52.49\% & 66.80\% \\
    Ours(DGCNN, B=0.6) & 73.86\% & \textbf{80.34\%} & 52.43\% & \textbf{68.95\%} \\
    \bottomrule
    \end{tabular}%
}
  \label{tab:ablation_PV_normal}%
\end{table}%
%%%%%%%% END Ablation

\noindent\textbf{Results \& Analysis.}  
As we can see from Table \ref{tab:ablation_normal}, the choice of LOP's structure has limited influence on the performance of PointRCNN under the normal circumstance. The differences between their precision are at most $1.49\%$, $0.72\%$ and $3.37\%$ on cars, pedestrians and cyclists, and the differences between their AP are at most $0.48\%$ on cars.
In contrast, the value of $B$ greatly affects the performance of PointRCNN.
Normally, the higher value of $B$ is realted with better performance of PointRCNN with the LOP: the precision of PointRCNN on cars and on cyclists increase with a larger $B$, while the change of AP on cars is always less than $2\%$. However, the LOP with a lower $B$ may bring PointRCNN better performance on detecting pedestrians, which is mainly because the larger precision of PointRCNN on pedestrians. As we can see from Fig.\ref{fig:ablation_atk}, although the LOP with the structure of DGCNN performs slightly better than the LOP with the structure of PointNet, the differences of the precision are always less than $3.48\%$, and the differences of the ASR are less than $4.00\%$ in most cases, a relatively small gap. Similarly, a higher $B$ always brings the better performance and the better defense effectiveness. For example, when $B=0.6$, the precision of PointRCNN with the LOP on cars increase \lyf{$10.79\%$ on} average, and the ASR of these appearing attacks decreases by $26.56\%$ on average compared with the results of $B=0.2$.
Besides, as we can see from Table \ref{tab:ablation_PP_normal}, Table \ref{tab:ablation_PV_normal} and Fig.\ref{fig:ablation_PPPV_atk}, the results is similar as the result on PointRCNN, which can further guarantee our analysis.

In fact, the point-wise PC model also performs well in other downstream tasks such as classification and semantic segmentation, which means the key features extracted by them is general enough to handle different CV tasks \cite{charles2017PN,charles2017PN++,yue2019DGCNN}. Thus, the LOP with different structures can both perform well in recognizing the components of real objects. However, in the pipeline of our proposed defense the value of $B$ directly determines whether a predicted object is preserved or eliminated. Therefore, the value of $B$ affects the performance of 3D object detectors equipped with the LOP.

Besides, as a trade-off, the increase in $B$ always causes the degradation in recall in the normal circumstances and under attacks. However, the degradation is limited by $10\%$ on average. Based on our discussion in Section \ref{sec:Limitation}, we consider it as a reasonable trade-off because the slight decrease in recall has limited influence on the normal function of ADS in the real word. In summary, the effectiveness of our proposed defense is insensitive to different choices of the model structure of LOP, while the value of $B$ does play an important role on the contrary. Regardless of the performance of the 3D object detectors in the normal circumstances and the acceptable trading of recall, the LOP with a higher $B$ can always bring the 3D object detector larger improvement.

==> tex/app_method.tex <==
\section{The Algorithm of Fake Object Elimination}
\label{appendix:FOE}
%%%%%% BEGIN OF ALGORITHM
\input{tex/alg/detection.tex}
%%%%%% END OF ALGORITHM 

==> tex/app_metrics.tex <==
\section{Two Popular Metrics to Evaluate PC Difference}
\label{appendix:metrics}

    \nonident \textbf{Chamfer Distance \cite{chong2019generating}.}
    \begin{align}
    D_C(S,S')= \frac{1}{||S'||}\sum_{y\in S'}min_{x\in S}||x-y||_2^2 \label{equal:chamfer}
    \end{align}
    \nonident \textbf{Average Square L2 Distance of kNN.}
    \begin{align}
    D_k(S,S')= \frac{1}{||S'||}\sum_{y\in S'}(\frac{1}{k}\sum_{x\in \text{kNN}(S,y)}||x-y||_2^2) \label{equal:knn}
    \end{align}
    In these equations, $S,S'$ denote two specific point sets defined above, $k$ denotes the hyper-parameter of $\text{kNN}(\cdot,\cdot)$ (we set $k=10$ in the following experiment), and $\text{kNN}(S,y)$ represents the $k$ nearest neighbor points of the point $y$ in the set $S$.
    % a subset of point set $S$, which includes $k$ nearest points of point $y$.

==> tex/app_mot.tex <==
\section{Multi-Object Tracking}
\label{appendix:mot}
Multi-object tracking (MOT) is a mid-level task, which grounds high-level tasks such as action recognition and behavior analysis, in computer vision \cite{wenhan2021motReview}. Usually, MOT can be divided into three small tasks: detecting multiple objects, maintaining their identities and tracking their trajectories separately. In ADS, the MOT module is always deployed between the perception module and the prediction module. Because the perception module has already provided the categories and locations of the objects nearby, the MOT module is mainly responsible for tracking their trajectories in essence \cite{xinshuo2020AB3DMOT,hsu2021P3DMOT}.

More specifically, the MOT module usually takes the predictions generated by the perception module as input, and matches these predicted objects with its maintained object trajectories. For those matched predicted objects and object trajectories, the MOT module uses a Kalman Filter (KF) or its variants to update each object trajectory based on its corresponding predicted object. For those unmatched predicted objects and object trajectories, the MOT module creates new object trajectories for some predicted objects, and removes some overdue object trajectories according to the predefined heuristic rules. Finally, the MOT module sends its maintained object trajectories to the prediction module for predicting the future movement of these objects and further analyzing.

==> tex/app_physicaleuipment.tex <==
\section{The General Physical Equipment for Appearing Attacks}
\label{appendix:physical_equipment}

%%%%%%%%%% BEGIN PHYSICAL DEVICE
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/physical_equipment.png}
    \caption{The physical equipment for appearing attacks.}
    \label{fig:appearing_attack_equipment}
\end{figure}
%%%%%%%%%%%% END PHYSICAL DEVICE


% \begin{table*}[t]
%   \centering
%   \caption{The results of hyper-parameter sensitive experiment on PointPillars and PV-RCNN in normal circumstance.}
% \scalebox{0.9}{
%     \begin{tabular}{rrrrrrr}
%     \toprule
%     \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{PointPillar} & \multicolumn{3}{c}{PV-RCNN} \\
% \cmidrule{2-7}    \multicolumn{1}{c|}{} & \multicolumn{1}{c}{Car} & \multicolumn{1}{c}{Pedestrian} & \multicolumn{1}{c|}{Cyclist} & \multicolumn{1}{c}{Car} & \multicolumn{1}{c}{Pedestrian} & \multicolumn{1}{c}{Cyclist} \\
%     \midrule
%     \multicolumn{1}{c|}{None} & \multicolumn{1}{c}{78.99\%} & \multicolumn{1}{c}{63.63\%} & \multicolumn{1}{c|}{59.11\%} & \multicolumn{1}{c}{73.12\%} & \multicolumn{1}{c}{53.34\%} & \multicolumn{1}{c}{62.17\%} \\
%     \midrule
%     \multicolumn{1}{c|}{Ours(PointNet, B=0.2)} & \multicolumn{1}{c}{80.12\%} & \multicolumn{1}{c}{63.99\%} & \multicolumn{1}{c|}{60.09\%} & \multicolumn{1}{c}{74.83\%} & \multicolumn{1}{c}{54.14\%} & \multicolumn{1}{c}{62.91\%} \\
%     \multicolumn{1}{c|}{Ours(PointNet, B=0.3)} & \multicolumn{1}{c}{80.46\%} & \multicolumn{1}{c}{64.00\%} & \multicolumn{1}{c|}{59.91\%} & \multicolumn{1}{c}{75.49\%} & \multicolumn{1}{c}{\textbf{54.16\%}} & \multicolumn{1}{c}{63.30\%} \\
%     \multicolumn{1}{c|}{Ours(PointNet, B=0.4)} & \multicolumn{1}{c}{81.04\%} & \multicolumn{1}{c}{\textbf{64.27\%}} & \multicolumn{1}{c|}{61.34\%} & \multicolumn{1}{c}{76.50\%} & \multicolumn{1}{c}{53.80\%} & \multicolumn{1}{c}{63.17\%} \\
%     \multicolumn{1}{c|}{Ours(PointNet, B=0.5)} & \multicolumn{1}{c}{81.77\%} & \multicolumn{1}{c}{63.45\%} & \multicolumn{1}{c|}{61.50\%} & \multicolumn{1}{c}{77.85\%} & \multicolumn{1}{c}{53.13\%} & \multicolumn{1}{c}{63.13\%} \\
%     \multicolumn{1}{c|}{Ours(PointNet, B=0.6)} & \multicolumn{1}{c}{\textbf{82.38\%}} & \multicolumn{1}{c}{63.47\%} & \multicolumn{1}{c|}{\textbf{62.11\%}} & \multicolumn{1}{c}{\textbf{78.53\%}} & \multicolumn{1}{c}{53.00\%} & \multicolumn{1}{c}{\textbf{64.99\%}} \\
%     \midrule
%     \multicolumn{1}{c|}{Ours(DGCNN, B=0.2)} & \multicolumn{1}{c}{80.88\%} & \multicolumn{1}{c}{64.71\%} & \multicolumn{1}{c|}{60.44\%} & \multicolumn{1}{c}{76.43\%} & \multicolumn{1}{c}{\textbf{54.40\%}} & \multicolumn{1}{c}{63.94\%} \\
%     \multicolumn{1}{c|}{Ours(DGCNN, B=0.3)} & \multicolumn{1}{c}{81.41\%} & \multicolumn{1}{c}{64.42\%} & \multicolumn{1}{c|}{60.51\%} & \multicolumn{1}{c}{77.04\%} & \multicolumn{1}{c}{51.16\%} & \multicolumn{1}{c}{64.35\%} \\
%     \multicolumn{1}{c|}{Ours(DGCNN, B=0.4)} & \multicolumn{1}{c}{82.20\%} & \multicolumn{1}{c}{\textbf{64.73\%}} & \multicolumn{1}{c|}{63.56\%} & \multicolumn{1}{c}{78.30\%} & \multicolumn{1}{c}{53.77\%} & \multicolumn{1}{c}{64.93\%} \\
%     \multicolumn{1}{c|}{Ours(DGCNN, B=0.5)} & \multicolumn{1}{c}{83.04\%} & \multicolumn{1}{c}{64.42\%} & \multicolumn{1}{c|}{64.89\%} & \multicolumn{1}{c}{79.61\%} & \multicolumn{1}{c}{52.49\%} & \multicolumn{1}{c}{66.80\%} \\
%     \multicolumn{1}{c|}{Ours(DGCNN, B=0.6)} & \multicolumn{1}{c}{\textbf{83.90\%}} & \multicolumn{1}{c}{64.44\%} & \multicolumn{1}{c|}{\textbf{66.45\%}} & \multicolumn{1}{c}{\textbf{80.34\%}} & \multicolumn{1}{c}{52.43\%} & \multicolumn{1}{c}{\textbf{68.95\%}} \\
%     \midrule
%           &       &       &       &       &       &  \\
%     \end{tabular}%
% }
%   \label{tab:ablation_PPPV_normal}%
% \end{table*}%

As shown in Fig.\ref{fig:appearing_attack_equipment}, a general physical equipment for appearing attacks consists of several photodiodes, a delay component and several combinations of laser transmitters and lens. Usually, the photodiode is responsible for beginning the attack. Once the photodiode receives the lasers emitted by the victim ADS's LiDAR, it generates the current and activates the delay component.
The delay component then controls the laser transmitter to emit lasers to the LiDAR and injects points into the PC generated by the LiDAR. Because the delay component can determine the time of flight of emitted lasers, the laser transmitter can determine the light intensity of emitted lasers, and the lens can determine the direction of emitted lasers, the attacker is possible to inject a certain number of points within a certain area as he/she wishes.



==> tex/app_realworld.tex <==
\section{Experiment on Real-world Data}
\label{app:realworld}
\noindent\textbf{Experiment Settings.}  We also evaluate the effectiveness of our defense with an experimental vehicle for automated driving, the D-KIT Advanced \cite{DKit} (Fig.\ref{fig:real_car}). Specifically, we collect the PCs captured by the Velodyne 128 LiDAR of the D-KIT Advanced when the ADS drives in a closed environment with ${5}$ moving obstacles. In detail, we gather $58$ frames of PCs from two independent driving tests (with different tracks) and annotate the ground-truth bounding boxes of the obstacles in the surrounding environment with the aid of the D-KIT Advanced. Next, we generate adversarial examples by the three appearing attacks we cover based on these clean samples. Then, we evaluate the performance of these 3D object detectors with and without the LOP. Table \ref{tab:real_pre} \& \ref{tab:real_asr} presents the precision of these 3D object detectors on cars and the ASR of the three attacks respectively.

%%%%%%% BEGIN REAL CAR
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{figs/real_car.png}
    \caption{The D-KIT Advanced which we use to gather the real-world PC data.}
    \label{fig:real_car}
\end{figure}
%%%%%%%% END REAL CAR


\begin{table}[ht]
  \centering
  % \vspace{-0.2in}
  \caption{The precision of 3D object detectors on cars with and without LOP on the real-world data.}
\scalebox{0.7}{
    \begin{tabular}{clccc}
    \toprule
          &       & \makecell{w/o. \\ defense}  & \makecell{Ours \\ (PointNet, B=0.5)} & \makecell{Ours \\ (DGCNN, B=0.5)} \\
    \midrule
    \multirow{3}[2]{*}{PointPillars} & w/o. attack  & 88.00\% & 89.47\% & \textbf{93.33\%} \\
          & Physical & 40.00\% & \textbf{65.22\%} & 57.14\% \\
          & Baseline  & 56.34\% & 61.76\% & \textbf{65.52\%} \\
    \midrule
    \multirow{4}[2]{*}{PointRCNN} & w/o. attack  & 98.39\% & \textbf{100.00\%} & \textbf{100.00\%} \\
          & Physical & 52.63\% & \textbf{71.11\%} & 59.52\% \\
          & Baseline  & 28.88\% & 74.00\% & \textbf{76.47\%} \\
          & Roadside & 16.39\% & \textbf{56.52\%} & 55.36\% \\
    \midrule
    \multirow{3}[2]{*}{PV-RCNN} & w/o. attack  & \textbf{100.00\%} & \textbf{100.00\%} & \textbf{100.00\%} \\
          & Physical & 24.59\% & \textbf{48.28\%} & 29.17\% \\
          & Baseline  & 14.43\% & \textbf{71.11\%} & 67.35\% \\
    \bottomrule
    \end{tabular}%
}
%   \vspace{-0.1in}
  \label{tab:real_pre}%
\end{table}%

\begin{table}[ht]
  \centering
  % \vspace{-0.2in}
  \caption{The ASR of implemented appearing attacks based on the real-world data.}
\scalebox{0.7}{
    \begin{tabular}{clccc}
    \toprule
          &       & \makecell{w/o. \\ defense}  & \makecell{Ours \\ (PointNet, B=0.5)} & \makecell{Ours \\ (DGCNN, B=0.5)} \\
    \midrule
    \multirow{2}[2]{*}{PointPillars} & Physical & 37.29\% & \textbf{8.47\%} & 13.56\% \\
          & Baseline  & 44.07\% & 16.95\% & \textbf{10.17\%} \\
    \midrule
    \multirow{3}[2]{*}{PointRCNN} & Physical & 76.27\% & \textbf{20.34\%} & 27.12\% \\
          & Baseline  & 15.25\% & \textbf{0.00\%} & 1.69\% \\
          & Roadside & 28.81\% & \textbf{3.39\%} & \textbf{3.39\%} \\
    \midrule
    \multirow{2}[2]{*}{PV-RCNN} & Physical & 67.80\% & \textbf{20.34\%} & 23.73\% \\
          & Baseline  & 1.69\% & 1.69\% & \textbf{0.00\%} \\
    \bottomrule
    \end{tabular}%
}
% \vspace{-0.2in}
  \label{tab:real_asr}%
\end{table}%

\noindent\textbf{Results \& Analysis.} As we can see from Table \ref{tab:real_pre} and \ref{tab:real_asr}, our proposed defense also performs well in the real world. In the normal circumstances, the LOP can improve the performance of 3D object detectors, and their precision can reach $100\%$ in most cases. Furthermore, the 3D object detectors with LOP can limit the ASR of appearing attacks less than $20\%$ in most cases, even decrease the ASR of Baseline which aims at PointRCNN and PV-RCNN to $0\%$. 
Although the performance of LOP in the real world can not compare with that on the KITTI dataset, we argue it is mainly because the real-world scenes sampled by us are different from the scenes present in the KITTI dataset, that these real-world scenes contain more stationary objects which are not considered in the prediction of these 3D object detectors. In other words, these objects are natural noises to the 3D object detector, and may harm their performance.
In summary, our proposed defense can not only defend against appearing attacks, but also improve the performance of 3D object detectors in the real world.

==> tex/app_stage3code.tex <==
\section{Pseudo-Code of Fake Object Elimination}
\label{appendix:stage3_code}

%%%%%% BEGIN OF ALGORITHM
\input{tex/alg/detection.tex}
%%%%%% END OF ALGORITHM 

The Alg.\ref{alg:detecting} shows the process of the fake object elimination stage in the pipeline of our proposed defense.

==> tex/app_sys.backup.tex <==
Specifically, we selected 5 different fake PCs based on the previous experiments which are located in front of the self-driving vehicle in 10 meters and can successfully forged the perception module of Apollo for at least one frame. Meanwhile, we use Apollo to record 3 different traces of the self-driving vehicle moving under manually control. Then, we inject these fake PCs into all the frames of these traces to generate 15 different fully poisoned traces. During the experiments, we run Apollo 6.0.0 system with and without LOP on these traces and visualize the future routes generated by the planning module of Apollo (which is also shown as a green rectangle in front of the self-driving vehicle) in the Dreamview, and assume there is a car moving behind the self-driving vehicle at a constant speed. Based on the generated future route, we can determine whether the self-driving vehicles will suddenly brake if they are controlled by the Apollo system, and consider the brake as a potential crash.

As shown in the part (a) of Fig.\ref{fig:sys_level_apollo}, the generated future route is extended to the crossroads, which means the self-driving vehicle will moving normally and stop at a red light under the instructions of the Apollo with our LOP. Therefore, we consider this situation as ``no accident''. Meanwhile, as shown in the part (b) of Fig.\ref{fig:sys_level_apollo}, the generated future route disappears for a while, which means the self-driving vehicle will falsely stop in the middle of the road and hit by the potential car moving behind it. Therefore, we consider this situation as ``car crash''. The crash rate we report in the Section 5.4 are calculated based on the number of ``car crash'' in the 15 poisoned traces above.

==> tex/backup/0_backup_ourmethod.tex <==
\section{Our Defense: Local Objectness Detector}\label{sec:OurDefense}
\subsection{Insight of Existing Appearing Attacks}
Though these existing appearing attacks differ from one another in various aspect, we find that there are two common properties of them.

\subsubsection{Property 1: Inimitable Relation between Features}
Because most of existing appearing attacks focus on being a real threat in the real world, they are inevitably limited by attacker's goal and physical equipment: as we describe in Sec.\ref{sec:Limitation}, there are upper bounds for the number of added points and the distance between a fake object and LiDAR. Behind these two limitations, there is an unsolved problem remained for existing appearing attacks: with current method, it is hard to imitate the relation between the \textit{depth}, i.e. the distance between a object and the LiDAR, and the \textit{point density}, i.e. the ratio of the number of input points inside a object's bounding box over the volume of this bounding box, of a real object in the real world.

% Potential Graph: distribution of real objects and fake objects in a depth-density graph

Thus, we adopt a PC classifier to learn the relation between the depths and the point densities of real objects under different situation, and distinguish real objects and fake objects based on this relation.

\subsubsection{Property 2: Unnoticed Local Difference}
Except the category and the bounding box, 3D object detectors will also calculate a confidence score or an objectness score for each predicted object to quantify whether it is real into a numerical value. 3D object detectors in essence return the objects with higher scores as its final prediction. Therefore, most of existing appearing attacks focus on increasing the objectness score of fake objects, while they ignore the difference between the local part of real objects and fake objects.

% Potential Graph: local difference is much larger than the global difference

Besides, Chen's work has showed that with an appropriate strategy of spatial division, one single part of real objects contains enough spatial information and semantic information to predict the category, the bounding box and the objectness score of its related object\cite{qi2020object}. Thus, we split the input space into several equal-size pillars and predict whether the input points inside represented a part of a real object for each pillar. For each predicted objects, we choose the pillars intersected with its bounding box, and determine whether the predicted object is a real object by voting.

\subsection{Local Objetness Detector}
\subsubsection{Overview}
Based on the two common properties of existing appearing attacks, we propose a local objectness detector to determine whether a object in prediction is real or not. As shown in Fig.\ref{fig:local_objectness_detector}, the pipeline of our local objectness detector can be divided into three stages: sample Generating stage, training stage and detecting stage.

\begin{figure*}[htpb]
    \centering
    \includegraphics[width=2\columnwidth]{figs/placeholder.png}
    \caption{The pipeline of our local objectness detector.}
    \label{fig:local_objectness_detector}
\end{figure*}

\subsubsection{Sample Generating Stage}
At this stage, we focus on generating training set, which is based on the original training set of target 3D object detector without any auxiliary information, for our local objectness detector. 

For each sample in the original training set, we divide the input space into several equal-size pillars, which are equal to $1m\times1m$ grids in the x-y plane. We then turn each pillar with points inside into a training sample based on following ways:

\paragraph{Generating Feature} For each point inside this pillar, we first turn its $4$-dim feature vector $(x,y,z,int)$ into a $7$-dim feature vector$(dx,dy,x,y,z,int,dep)$, where $(x,y,z)$ is its 3D coordinates, $(dx,dy)$ is its 2D relative coordinates to the center of this pillar in x-y plane, $int$ is its intensity and $dep=\sqrt{x^2+y^2+z^2}$ is its depth. We then concatenate these new feature vectors to generate the feature tensor of size $(M,7)$, where $M$ is a fixed super-parameter\footnote{We choose $M=1024$ in our experiment.}. For those pillar with more than $M$ points inside, we randomly sample $M$ points; for those pillar with less than $M$ points inside, we apply zero padding.

\paragraph{Generating Label} We calculate the 2D Intersection over Union (IoU), the IoU on the x-y plane, of this pillar and each bounding box of the ground truth in original training sample, and store the max IoU over them. If the max IoU is greater than a fixed threshold $\alpha$, then we consider there is a part of real object including in this pillar and set 1 as its label\footnote{We choose $\alpha=1e^{-6}$ in our experiment.}. Otherwise, we set 0 as its label.

Finally, we collect all pairs of (feature, label) as the training set for our local objectness detector.

However, the \textit{positive samples}, i.e. the generated samples with 0 as label, are much more than the \textit{negative samples}, i.e. the generated samples with 1 as label. To keep data balance, we delete a part of negative samples in random to ensure that the ratio of positive samples and negative samples does not exceed $1:1.5$.

\subsubsection{Training Stage}
Due to the good performance of point-wise PC models on various 3D tasks, we implement a point-wise PC classifier as our local objectness detector. We choose Adam with learning rate $=1e^{-3}$ as the optimizer and focal loss as the loss function:

\begin{align}
FL(p,y)=-\alpha(1-p_y)^\gamma log(p_y) \label{equal:3}
\end{align}

where $\alpha,\gamma$ are super-parameters, $p$ is the probability vector returned by classifier and $y$ is the label of input data\footnote{We choose $\alpha=1,\gamma=2$ in our experiments.}. Finally, we train our local objectness detector on our collected training set until its convergence.

\subsubsection{Detecting Stage}
To identify the fake objects in prediction, we first divide the detection space into several equal-size pillars and generate their features similarly to the sample generating stage. Then we use our local objectness detector to generate $0/1$ objectness score for each pillar. 

For each object in the prediction, we find the pillars that the 2D IoU between them and the bounding box of this object is greater than a specified threshold $\beta$ and count the sum of their objectness scores\footnote{We choose $\beta=1e^{-3}$ in our experiment.}. Finally, we recognize the objects with the ratio of this sum over the number of counted pillars equal to or less than $50\%$ as fake objects and erase them from the prediction.

==> tex/backup/backup_abs_xqf.tex <==
\begin{abstract}
Modern self-driving systems mainly rely on object detectors, especially LiDAR-based (Light Detection and Ranging) 3D object detectors, to perceive the objects nearby autonomous vehicles. However, some adversarial attacks such as appearing attack have been proved threat to AV, because it can forge inexistent objects for 3D object detectors and further cause traffic accidents. Existing defenses remove suspect points or objects based on their statistical features, which have limitations in their performances and generalizations. In this work, we propose a local objectness detectors to distinguish the local difference between the fake objects and the real objects and avoid appearing attacks. We design our local objectness detectors based on two common properties of existing appearing attacks revealed by us. First, most existing appearing attacks are limited by attacker's goal and attacker's capability. Behind these limitations, there is an invariant relation between the depth and the point density of real objects. Second, most existing appearing attacks focus on forging the fake object which is similar as a real object in general, regardless of the local difference between them. We further deploy our local objectness detectors on three state-of-the-art 3D object detectors and evaluate these object detectors' performances. 
The results show that our local objectness detectors can increase 3D object detectors' precisions from $28\sim66\%$ to $60\sim74\%$ under appearing attacks.
% The results show that our local objectness detectors can increase 3D object detectors' precisions from $[data0]!!!$ to $[data1]!!!$ under appearing attacks.

% data0->不防御的情况下，受攻击的3D实体检测模型的precision范围
% data1->防御的情况下，受攻击的3D实体检测模型的precision范围


% 摘要提纲：
% 1、自动驾驶系统依赖3D实体检测模型基于点云检测周围的实体，但现在已经证明了对抗性攻击可以有效攻击3D实体检测模型
% 2、appearing attack作为其中一种对抗性攻击，能导致3D实体检测模型检测到不存在的实体，进而导致自动驾驶小车紧急制动造成交通阻塞甚至是追尾事故
% 3、现有的防御研究都是针对其中一种或几种appearing attack设计，缺乏泛化性
% 4、我们研究了现存的几种appearing attack，发现了它们所具有的相同特点，并利用这一点设计了防御appearing attack的伪造实体检测模型。
% 5、我们通过实验发现，使用了我们的伪造实体检测模型后，3D实体检测模型的precision在无攻击场景和有攻击场景中都明显提升
\end{abstract}

==> tex/backup/backup_experiment_xqf.tex <==
\section{Experiments} \label{sec:Experiment}
In this section, we deploy our local objectness predictor on three state-of-the-art 3D object detectors to evaluate their performances in normal circumstances \louis{as well as} under appearing attacks. Besides, we further compare the defense effect of our local objectness predictor with other existing defenses against appearing attacks. Below, we describe the setup of experiments and report the results.

\subsection{Setup}\label{sec:Experiment:setup}
\paragraph{Victim 3D Object Detectors} We choose Pointpillars \cite{alex2019pointpillars}, PointRCNN \cite{shaoshuai2019pointrcnn} and PV-RCNN \cite{shaoshuai2020pvrcnn} as the victim 3D object detectors. We adopt the \louis{pre-trained} 3D object detectors, which are trained on the KITTI dataset \cite{andreas2012kitti}, supported by OpenPCDet\footnote{https://github.com/open-mmlab/OpenPCDet/}, an open-source testing platform for 3D object detection. Because these 3D objects detectors may return some objects with a low confidence score in prediction, which may significantly injure their performance, we only consider the objects with confidence scores larger than a threshold $C$ in their prediction to keep their precision in a normal level. For Pointpillars and PointRCNN, we set $C=0.5$; for PV-RCNN, we set $C=0.7$.

\paragraph{Attack Methods} We implement following three different appearing attacks to deceive the victim 3D object detectors:
\begin{itemize}
    \item \textbf{the Variant of Adv-LiDAR \cite{yulong2019advSensor}} Because Adv-LiDAR is specially designed for the LiDAR-based 3D object detector of Baidu's Apollo, it is unsuitable to directly implement it to attack other 3D object detectors. Thus, we follow Adv-LiDAR's idea and propose the variant of ADV-LiDAR: randomly inject a certain amount of the points into a specified zone, and use FGSM to increase the confidence scores of those fake object related to these points.
    \item \textbf{Sun's Work \cite{jiachen2020towards}} This attack forge objects by duplicating the real objects with limited points and transforming them to the position near the victim autonomous vehicle. 
    \item \textbf{Yang's Work \cite{kaichen2021robust}} This attack forge objects by increasing the confidence scores of fake objects and enlarging their bounding boxex with gradient descent  methods \footnote{In the original paper, this attack mainly aim at PointRCNN in the white-box scenario. We follow this settings in our experiments.}.
\end{itemize}

\paragraph{Other Defense Methods} \louis{Besides} our LOP, we also implement SRS, SOR and CARLO as comparison. The details of these defense methods are introduced in Sec.\ref{sec:Limitation}. Especially, due to the large time cost and computation of deploying SVF and re-training the victim 3D object detectors, we do not evaluate the effect of SVF in the experiments. Besides, CARLO and SVF are specially designed for the same appearing attack, thus we believe the results of CARLO can be representative of SVF in a certain extent.

\subsection{Results}\label{sec:Experiment:results}
\subsubsection{Without Attacks}\label{sec:Experiment:results:woAtk}
\noindent\textbf{Experiment Settings.} We first evaluate the performance of our LOP in normal circumstance. We implement our LOP on three state-of-the-art 3D object detectors, and evaluate their precision on the validating samples of KITTI dataset. Without loss of generality, we choose two different point-wise PC classifier, PointNet and DGCNN, as the our LOP, and choose five different values as the boundary values $B$ of our LOP. Table \ref{tab:normal_pre} presents the precision of these 3D object detectors in normal circumstance.

\begin{table*}[htbp]
  \centering
  \caption{The precision of 3D object detectors with and without LOP on clean samples. "PointNet" and "DGCNN" refers to the model structure of our LOP, and $B$ is the boundary value of our LOP, which is used to distinguish real objects and forged objects as the description in Sec.\ref{sec:method:voting}.}
\scalebox{0.9}{
    \begin{tabular}{c|ccc|ccc|ccc}
    \toprule
    % Model 
    & \multicolumn{3}{c|}{PointPillar} & \multicolumn{3}{c|}{PointRCNN} & \multicolumn{3}{c}{PV-RCNN} \\
    \cmidrule{2-10}
    % Object Type 
    & Car   & pedestrian & Cyclist & Car   & pedestrian & Cyclist & Car   & pedestrian & Cyclist \\
    \midrule
    None  & 78.99\% & 63.63\% & 59.11\% & 75.04\% & 47.08\% & 56.87\% & 73.12\% & 53.34\% & 62.17\% \\
    \midrule
    % Ours(PointNet, B=0.2) & 80.12\% & 63.99\% & 60.09\% & 76.49\% & 50.70\% & 58.66\% & 74.83\% & 54.14\% & 62.91\% \\
    % Ours(PointNet, B=0.3) & 80.46\% & 64.00\% & 59.91\% & 77.15\% & \textbf{50.94\%} & 58.93\% & 75.49\% & \textbf{54.16\%} & 63.30\% \\
    Ours(PointNet, B=0.4) & 81.04\% & \textbf{64.27\%} & 61.34\% & 78.05\% & \textbf{50.49\%} & 61.59\% & 76.50\% & \textbf{53.80\%} & 63.17\% \\
    Ours(PointNet, B=0.5) & 81.77\% & 63.45\% & 61.50\% & 79.29\% & 49.63\% & 61.92\% & 77.85\% & 53.13\% & 63.13\% \\
    Ours(PointNet, B=0.6) & \textbf{82.38\%} & 63.47\% & \textbf{62.11\%} & \textbf{80.03\%} & 49.43\% & \textbf{63.87\%} & \textbf{78.53\%} & 53.00\% & \textbf{64.99\%} \\
    \midrule
    % Ours(DGCNN, B=0.2) & 80.88\% & 64.71\% & 60.44\% & 77.56\% & 51.04\% & 61.03\% & 76.43\% & \textbf{54.40\%} & 63.94\% \\
    % Ours(DGCNN, B=0.3) & 81.41\% & 64.42\% & 60.51\% & 78.36\% & \textbf{51.31\%} & 61.72\% & 77.04\% & 51.16\% & 64.35\% \\
    Ours(DGCNN, B=0.4) & 82.20\% & \textbf{64.73\%} & 63.56\% & 79.44\% & \textbf{51.21\%} & 63.74\% & 78.30\% & \textbf{53.77\%} & 64.93\% \\
    Ours(DGCNN, B=0.5) & 83.04\% & 64.42\% & 64.89\% & 80.75\% & 49.59\% & 65.14\% & 79.61\% & 52.49\% & 66.80\% \\
    Ours(DGCNN, B=0.6) & \textbf{83.90\%} & 64.44\% & \textbf{66.45\%} & \textbf{81.52\%} & 49.42\% & \textbf{67.24\%} & \textbf{80.34\%} & 52.43\% & \textbf{68.95\%} \\
    \bottomrule
    \end{tabular}
}
  \label{tab:normal_pre}
\end{table*}

\noindent\textbf{Result \& Analysis.} As we can see from Table \ref{tab:normal_pre}, these three 3D objectors detectors all benefit from our LOP: their precision on cars increase $1.13\sim7.12\%$ with our LOP, and their precision on cyclists increase $0.74\sim10.37\%$ with our LOP. Though their precision on pedestrians may degrade due to our LOP, the scale of degradation is at most $2.18\%$, which is far less than the improvement LOP bring in other aspects. We believe that there are two reasons caused the degradation of precision on pedestrians. On the one hand, the point density and the depth of pedestrians are usually less than cars and cyclists. It increases the difficulty of the depth-density relation modeling, which is the key to the performance of our LOP. On the other hand, the performance of 3D object detectors on pedestrians are usually worse than their performance on cars and cyclists due to the difficulty of recognizing small objects, which increases the difficulty of distinguish real objects and forged objects for our LOP. Besides, existing appearing attacks focus on forging car, so it is not necessary to implement LOP to eliminate forged pedestrians. As a summary, our LOP can increase the performance of 3D object detectors in most aspects, and there also exists valid way to avoid the latent damage caused by our LOP.

\subsubsection{Under Attacks}\label{sec:Experiment:results:uAtk}
\noindent\textbf{Experiment Settings.} Next, we evaluate the performance of our LOP against existing appearing attacks. We follow the settings in Sec.\ref{sec:Experiment:results:woAtk}, and implement three existing appearing attacks to generate adversarial samples based on the validating samples of KITTI dataset. We then evaluate the attack success rate (ASR) of forged objects and the precision of the 3D object detectors on these adversarial samples \footnote{Besides the forged objects crafted by appearing attacks, there also remains some normal objects in adversarial samples.}. Table \ref{tab:attack_asr} shows the ASR of three existing appearing attacks on 3D object detectors, and Table \ref{tab:attack_pre} presents the precision of three different 3D object detectors under existing appearing attacks.

\begin{table*}[htbp]
  \centering
  \caption{The precision of 3D object detectors with and without LOP on adversarial samples. "None" refers to no attack, "Physical" refers to the black-box appearing attack proposed in Sun's work, "FGSM" refers to the variant of Adv-LiDAR , and 'Roadside' refers to the white-box appearing attack proposed in Yang's work. Here, three attacks are described in Sec.\ref{sec:Experiment:setup} in details.}
\scalebox{0.9}{
    \begin{tabular}{c|ccc|cccc|ccc}
    \toprule
          & \multicolumn{3}{c}{PointPillar} & \multicolumn{4}{c|}{PointRCNN} & \multicolumn{3}{c}{PV-RCNN} \\
\cmidrule{2-11}          & None  & Physical & FGSM  & None  & Physical & FGSM  & Roadside & None  & Physical & FGSM \\
    \midrule
    None  & 78.99\% & 71.89\% & 66.61\% & 75.04\% & 61.82\% & 55.27\% & 50.47\% & 73.12\% & 64.06\% & 28.08\% \\
    \midrule
    % Ours(PointNet, B=0.2) & 80.12\% & 73.51\% & 69.06\% & 76.49\% & 64.65\% & 66.72\% & 62.65\% & 74.83\% & 66.11\% & 47.52\% \\
    % Ours(PointNet, B=0.3) & 80.46\% & 74.31\% & 70.12\% & 77.15\% & 66.40\% & 68.77\% & 65.32\% & 75.49\% & 67.35\% & 50.23\% \\
    Ours(PointNet, B=0.4) & 81.04\% & 75.79\% & 72.08\% & 78.05\% & 69.14\% & 71.33\% & 68.80\% & 76.50\% & 69.20\% & 54.58\% \\
    Ours(PointNet, B=0.5) & 81.77\% & 77.65\% & 74.60\% & 79.29\% & 73.09\% & 74.33\% & 72.87\% & 77.85\% & 72.82\% & 60.33\% \\
    Ours(PointNet, B=0.6) & \textbf{82.38\%} & \textbf{79.23\%} & \textbf{76.08\%} & \textbf{80.03\%} & \textbf{75.45\%} & \textbf{76.13\%} & \textbf{74.99\%} & \textbf{78.53\%} & \textbf{74.69\%} & \textbf{61.17\%} \\
    \midrule
    % Ours(DGCNN, B=0.2) & 80.88\% & 74.33\% & 69.91\% & 77.56\% & 64.84\% & 69.06\% & 65.58\% & 76.43\% & 67.07\% & 51.25\% \\
    % Ours(DGCNN, B=0.3) & 81.41\% & 75.47\% & 71.30\% & 78.36\% & 66.91\% & 71.23\% & 68.45\% & 77.04\% & 68.46\% & 54.11\% \\
    Ours(DGCNN, B=0.4) & 82.20\% & 77.23\% & 73.51\% & 79.44\% & 69.85\% & 73.86\% & 72.28\% & 78.30\% & 71.00\% & 58.57\% \\
    Ours(DGCNN, B=0.5) & 83.04\% & 79.18\% & 76.10\% & 80.75\% & 73.83\% & 76.60\% & 75.83\% & 79.61\% & 74.19\% & 63.49\% \\
    Ours(DGCNN, B=0.6) & \textbf{83.90\%} & \textbf{80.83\%} & \textbf{78.08\%} & \textbf{81.52\%} & \textbf{75.92\%} & \textbf{78.11\%} & \textbf{77.66\%} & \textbf{80.34\%} & \textbf{75.99\%} & \textbf{64.30\%} \\
    \bottomrule
    \end{tabular}
}
  \label{tab:attack_pre}
\end{table*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/ASR_single.png}
    \caption{The ASR of three appearing attacks on different 3D object detectors with and without LOP.}
    \label{fig:asr_single}
\end{figure}

\noindent\textbf{Result \& Analysis.} As we can see from Fig. . 

\subsubsection{Compared with Other Defenses}\label{sec:Experiment:results:comp}
Furthermore, we compare the performance of our LOP with other existing defense methods in normal circumstance and under attacks. We implement three existing appearing attacks to generate adversarial samples based on the validating samples of KITTI dataset. Table [TODO:precision] presents the precision of three different 3D object detectors in normal circumstance, and Table [TODO:precision] presents the precision of three different 3D object detectors under appearing attacks.

\begin{table*}[htbp]
  \centering
  \caption{The precision of 3D object detectors with different defenses on clean samples. $M$, $K$ and $r$ refers to the super-parameters of these three defenses which is introduced in Sec.\ref{sec:Limitation} in details.}
\scalebox{0.9}{
    \begin{tabular}{c|ccc|ccc|ccc}
    \toprule
          & \multicolumn{3}{c|}{PointPillar} & \multicolumn{3}{c|}{PointRCNN} & \multicolumn{3}{c}{PV-RCNN} \\
\cmidrule{2-10}          & Car   & pedestrian & Cyclist & Car   & pedestrian & Cyclist & Car   & pedestrian & Cyclist \\
    \midrule
    None  & 78.99\% & 63.63\% & 59.11\% & 75.04\% & 47.08\% & 56.87\% & 73.12\% & 53.34\% & 62.17\% \\
    SRS (M=500) & 79.14\% & 63.22\% & 59.24\% & 74.75\% & 51.00\% & 56.34\% & 73.23\% & 53.50\% & 63.82\% \\
    \midrule
    SOR (k=2) & 78.91\% & 62.40\% & 58.44\% & 74.49\% & 45.46\% & 55.72\% & 72.92\% & 52.62\% & 61.95\% \\
    SOR(k=10) & 78.86\% & 61.60\% & 58.00\% & 73.88\% & 44.05\% & 55.32\% & 72.94\% & 52.18\% & 60.57\% \\
    \midrule
    CARLO(LPD, r=0.6) & 75.06\% & 6.37\% & 12.64\% & 73.10\% & 10.23\% & 15.23\% & 70.08\% & 7.46\% & 14.29\% \\
    CARLO(LPD, r=0.7) & 77.81\% & 11.99\% & 19.94\% & 74.35\% & 15.85\% & 22.64\% & 72.22\% & 13.03\% & 22.50\% \\
    CARLO(LPD, r=0.8) & 78.00\% & 21.40\% & 27.12\% & 74.32\% & 23.26\% & 29.00\% & 72.41\% & 20.56\% & 28.59\% \\
    \midrule
    CARLO(FSD, r=0.6) & 75.77\% & 39.47\% & 41.75\% & 73.07\% & 35.44\% & 38.46\% & 69.93\% & 36.78\% & 40.92\% \\
    CARLO(FSD, r=0.7) & 77.56\% & 53.27\% & 55.38\% & 74.38\% & 42.22\% & 54.21\% & 71.66\% & 47.34\% & 58.50\% \\
    CARLO(FSD, r=0.8) & 78.31\% & 63.29\% & 58.25\% & 74.87\% & 46.87\% & 56.81\% & 72.37\% & 53.07\% & 61.44\% \\
    \midrule
    Ours(PointNet, B=0.5) & 81.77\% & 63.45\% & 61.50\% & 79.29\% & \textbf{49.63\%} & 61.92\% & 77.85\% & \textbf{53.13\%} & 63.13\% \\
    Ours(PointNet, B=0.6) & 82.38\% & 63.47\% & 62.11\% & 80.03\% & 49.43\% & 63.87\% & 78.53\% & 53.00\% & 64.99\% \\
    Ours(DGCNN, B=0.5) & 83.04\% & 64.42\% & 64.89\% & 80.75\% & 49.59\% & 65.14\% & 79.61\% & 52.49\% & 66.80\% \\
    Ours(DGCNN, B=0.6) & \textbf{83.90\%} & \textbf{64.44\%} & \textbf{66.45\%} & \textbf{81.52\%} & 49.42\% & \textbf{67.24\%} & \textbf{80.34\%} & 52.43\% & \textbf{68.95\%} \\
    \bottomrule
    \end{tabular}%
}
  \label{tab:addlabel}%
\end{table*}%

[TODO:Table and Result Analyze]

\subsection{Simulated Driving Test}\label{sec:Experiment:results:simulation}
\noindent\textbf{Experiment Settings.} [TODO]

[TODO]

\noindent\textbf{Result \& Analysis.} [TODO]


==> tex/backup/backup_intro.tex <==
\section{Introduction}\label{sec:Introduction}
Due to the rapid development of deep learning, several safety-critical applications have adopted deep neural networks (DNNs) to improve their performances \cite{edward2016doctorai,jiaxuan2019anAutomated}. As one of the safety-critical applications, autonomous vehicles also benefit from it by deploying different DNNs in their self-driving systems, e.g., implementing object detectors in the perception modules to predict the category and the location of each object around autonomous vehicles \cite{yulong2019advObj,gregory2019lasernet}. Because the point clouds (PCs) generated by LiDARs (Light Detection and Ranging) contains richer location information than the images generated by cameras, most existing self-driving systems, such as Baidu's Apollo Go\footnote{https://apollo.auto/} and Google's Waymo One\footnote{https://waymo.com/waymo-one/}, set LiDARs as the main sensors and rely on the predictions of \textit{3D object detectors} \cite{alex2019pointpillars,shaoshuai2019pointrcnn,shaoshuai2020pvrcnn,gregory2019lasernet}, one kind of models which take PCs as models' inputs and predicts the category and the location of each object nearby.

However, recent works find that these LiDAR-based object detectors in autonomous vehicles are vulnerable to some \textit{adversarial attacks} \cite{yulong2019advObj,kaichen2021robust}, which changes the predicted category or location of 3D object detectors by perturbing original points or adding new points in the input PCs, i.e. appearing attacks. Appearing attacks aim at forging inexistent vehicles in detectors' predictions, which may cause the emergency braking, and further lead to some serious threats such as the traffic jam or the crash accident in the real world  \cite{hocheol2017illusion,yulong2019advSensor,jiachen2020towards}. Meanwhile, existing defense methods have limitations to defend against most existing appearing attacks, which will be introduced in Sec.\ref{sec:Limitation} in detailed.

\begin{figure}[htpb]
    \centering
    \includegraphics[width=\columnwidth]{figs/physical_equipment.png}
    \caption{The physical equipment for existing appearing attacks.}
    \label{fig:appearing_attack_equipment}
\end{figure}

\noindent\textbf{Our Work.} To generally defend against existing appearing attacks, we first summarize two important properties of existing appearing attacks. On the one hand, the limitations below restrict the effect of appearing attacks in the real world, and behind them there is the inimitable relation between the depth and the point density of real vehicles. In terms of the attacker's goal, the fake vehicles created by appearing attack have to be located nearby the victim autonomous vehicle. Otherwise, the victim will have enough time to re-route and bypass the fake vehicles. Consequently, the appearing attack may not lead to the real-world threats as the attacker wishes. Meanwhile, constraint to the attacker's physical equipment, which is a combination of a photodiode, a delay component, a laser transmitter and a lens shown in Fig. \ref{fig:appearing_attack_equipment}, the attacker can only forge limited amounts of points for appearing attack during one scan of the LiDAR. Therefore, it is impossible for the attackers fully copy the PC corresponding to a complete vehicle, and parse it nearby the victim by firing laser pulses.

On the other hand, the existing appearing attacks focus on increasing the objectness scores, which will directly affect the existence of objects in the 3D detector's predictions, of the fake vehicles. In other words, appearing attacks only imitate the fake vehicles as similar as the real vehicles in general, without caring about the local differences between them. Therefore, there remains distinguishable difference between the fake vehicles and the real vehicles in the local.

In this paper, we propose a local objectness predictor to predict the objectness scores, which represent the probability of a part of an object inside, for the divided, equal-sized space, e.g., voxels or pixels, of input space. We can thus distinguish the fake vehicles and the real vehicles by these objectness scores.

However, the depth-density relation is hard to model due to its complexity. For example, most of objects with smaller depth have larger point density, while those objects blocked by others have smaller depth and point density at the same time. Consequently, we re-generate input PCs’ feature vectors by explicitly embedding the depth of each point, which substantially improve the modeling capability compared with using the original input feature. Although, there are some defense methods such as CARLO and SVF \cite{jiachen2020towards} which are also proved effective by experiments, we argue that they are in essence heuristic algorithms based on point density. First, they are designed for one or several specific appearing attacks, while the generalization of them remains unproved. Besides, they haven't explicitly made use of the depth to distinguish real objects and fake objects.

Meanwhile, in the context of object detection, there is no explicit annotation for supervising the training of objectness detector. However, Chen et al. suggest that one single part of input space has already contained rich semantic information for a PC model to predict its related object's category and location \cite{qi2020object}. Inspired by their work, we construct the supervision task by taking the features of input points inside a pillar as input, and whether the pillar intersects with any bounding box of real objects as $0/1$ label. Technically, we use our local objectness predictor to predict objectness score for each pillar intersected with a predicted object's bounding box, and determine whether the object is real by voting of these objectness scores. 

Furthermore, we reveal that our local objectness predictor is model-agnostic: the performance of our local objectness predictor is robust to the change of the structure of itself or the structure of the 3D object detector. From this perspective, our local objectness predictor is more effective than the traditional defense methods.

To understand the impact of our defense, we further implement most existing appearing attacks against three start-of-the-art 3D object detectors: PointPillars \cite{alex2019pointpillars}, PointRCNN \cite{shaoshuai2019pointrcnn} and PV-RCNN \cite{shaoshuai2020pvrcnn}. We compare their performance with and without our local objectness predictors, and find that: 
%with appearing attack, the detectors' precision can increase from $[data0]!!!$ to $[data1]!!!$ with our our local objectness predictors, while the detectors' precision can also increase from $[data2]!!!$ to $[data3]!!!$ with our our local objectness predictors in an un-attack situation.
with our our local objectness predictors, the 3D object detectors' precision on vehicles can increase from $28\sim66\%$ to $60\sim74\%$ under attack, while their precision on vehicles also increase from $73\sim79\%$ to $77\sim81\%$ in normal circumstances.
The results validate that our local objectness predictors can improve the robust of 3D object detectors to appearing attack without harming their normal performance.

% data0->不防御的情况下，受攻击的3D实体检测模型的precision范围
% data1->防御的情况下，受攻击的3D实体检测模型的precision范围
% data2->不防御的情况下，3D实体检测模型的正常precision范围
% data3->防御的情况下，3D实体检测模型的正常precision范围

\noindent\textbf{Our Contributions.} In summary, we mainly make the following key contributions:
\begin{itemize}
    \item We systematically inspect the existing appearing attacks and observe their common limitations. On the one hand, existing appearing attacks can't forge the relation between the depth and the point density of real vehicles. On the other hand, they mainly aim at increasing the confidence scores of the whole fake vehicles, regardless of the difference in small separated parts.
    \item Based on the discovery above, we propose a local objectness predictor as a general defense method for existing appearing attacks. Our local objectness predictor learns the depth-density relation of real objects, and discriminate the small parts of fake objects and real objects by predicting their objectness scores.
    \item We evaluate our defense against most existing appearing attacks on many start-of-the-art 3D object detectors, which strongly validates that our defense is efficient without side effects. For example, our local objectness predictors can increase a 3D object detectors' precision in normal circumstances or under attack, regardless of the structure of the 3D object detector.
\end{itemize}

==> tex/buffer/bank.tex <==
In contrast, in an appearing attack the attacker can choose the victim to fire the laser and forge non-existent cars as he/she wishes. Meanwhile, it is hard for others to notice this attack because there is almost no evidence left in the accident scene.

\xqf{Although due to the attack goal, it is meaningless to deploy LOP to defend against disappearing attacks, it is still worthwhile to evaluate the performance of LOP under mis-categorization attacks. We evaluate the performance of 3D object detectors under mis-categorization attacks in Appendix \ref{appendix:miscategorization}, and prove that LOP is also robustness against such attacks.}

% \noindent\textbf{Threats of Backdoor Attacks.}
\xqf{At last, }Backdoor attack is another threatening attack class to DNN models, which injects one or multiple backdoors into the victim model by modifying the training data \cite{chen2017targeted,turner2019labelconsitent}, the parameters \cite{jacob2020backdoorCNN,adnan2020TBT} or the network structure \cite{ruixiang2020embarrass}. After the injection, the adversary can activate his/her specified model misbehaviors by feeding special inputs containing the related trigger pattern. However, to implement a backdoor attack on the victim ADS is unrealistic. For example, the attacker requires the permission of the victim's self-driving system, which only belongs to a few administrators or security operators.


% On one hand, 
% to implement a disappearing attack, the attacker has to put the printed objects on the road or near some objects before the attack happens,
% which means the attack can not choose the victim ADS.
% On the other hand, after the first accident of disappearing attack, a printed object may be destroyed and the people nearby may realize that there is probably some problems with the printed object, so it is hard for the attacker to use the same printed object to cause the second accident.

% Besides, with such permission, the attacker is able to directly modify the outputs of any DNN models, or even any modules in the self-driving system.
% Besides, even with such permission, the attacker has no need to backdoor is able to modify any modules in the self-driving system, or even the outputs of DNN models directly.
% Therefore, we believe that it is hard for an attacker to acquire the permission, and,
% once getting the permission, the attacker does not need to implement such a backdoor attack because he/she can already manipulate the victim as his/her wish.

% If the input of target model doesn't activate any triggers, the target model will return the normal prediction as usual.
% Otherwise, the target model will return a specific prediction which is linked with the activated trigger by the attacker.

% In 2017, Chen et al. firstly apply backdoor attack in machine learning, and suggest a \louis{fixed-pattern} backdoor attack: the trigger in the target model will be activated by a fixed pattern in the input \cite{chen2017targeted}.
% Turner et al. suggest not to change the labels of backdoor samples \louis{added} into the target model's training set, and improve the invisibility of backdoor attack during the training stage of target model \cite{turner2019labelconsitent}.
% On the other hand, Li et al. and Pang et al. suggest dynamic-pattern backdoor attacks, where the trigger in the target model will be activated by different patterns for different inputs, and improve the invisibility of backdoor attack during the inference stage of target model \cite{li2019invisible,pang2020atale}.
% The studies above prove that backdoor attacks can manipulate the target model's output on specific tasks, without harming the model's performance on its main task or being noticed by others.


% he/she doesn't need to implement backdoor attack while he/she is able to manipulate the victim as his/her wish. 

% \noindent\textbf{Limitations and Future Directions.} 
% Although there may be potential adaptive attacks designed to break the LOP in the future, we argue that it is hard to implement in the real world. It is mainly because: 
% (i) Even the open-sourced ADS such as Apollo \cite{Apollo} keeps some small DNN models as black boxes. For example, there is a black-box DNN model used to locate the ADS in Apollo. The structure of this model is stored as an executable and linking file (*.so), and the parameter of this model is stored as an encrypted binary file (*.bin), which are difficult for attackers to decipher. Thus, it is also possible to protect the LOP by encrypting.
% (ii) The output of LOP is only a binary value to indicate the object is real or fake. Once the LOP is accessed as a black-box executable, it is generally hard for attacker to efficiently generate adversarial examples against our defense via optimization-based techniques.
% \morinop{(add discussion on adaptive attacks)}

==> tex/discussion_backup.tex <==
\section{Discussion}\label{sec:Discussion}
Our current defense mainly focuses on appearing attacks, which form a popular attack class on LiDAR-based object detectors in ADS. Below, we discuss other attack classes which may threaten the detector's security and why our current work chooses the appearing attack as the main research target.


\noindent\textbf{\xqf{Other Potential Attacks}} \xqf{Fisrt of all, }disappearing attacks on ADS also belong to the family of adversarial examples \cite{dawn2018physical,shang2018shapeshifter,yue2019seeing}.
\xqf{However, }different from appearing attacks, a disappearing attack aims at hiding the existing objects from the prediction results of the victim 3D object detector. To accomplish this purpose, in a disappearing attack the adversary usually generates an object by 3D printing, and puts it on the road or near some objects to conduct the attack. 
Technically, the specific shape of the printed object is optimally chosen to guarantee the target detector would not recognize it or its neighbouring object in the prediction results, leading to its disappearance in the detector's output.

In existing literature, Cao et al. propose the first disappearing attack on ADS, and successfully hide the printed objects from the LiDAR-based detection system of Baidu's Apollo by modeling its preprocessing and postprocessing phases into differentiable functions \cite{yulong2019advObj}.
Furthermore, Tu et al. suggest a more general disappearing attack which breaks the state-of-the-art 3D object detectors including PointPillars and PointRCNN, and hide the car on which the printed object is positioned from the model's prediction results \cite{james2020physically}.
Recently, Cao et al. suggest a more powerful disappearing attack, MSF-ADV, which fools the image-based 2D object detectors and LiDAR-based 3D object detectors at the same time, and causes the fusion-based detection system of Baidu's Apollo to ignore the existence of the printed objects \cite{yulong2021invisible}.

\xqf{Besides, mis-categorization attacks are also one of the threatening adversarial attacks to ADS. A mis-categorization attack can be seen as the combination of a disappearing attack and a appearing attack, it aims at changing the predicted class of the target objects in the prediction results of the victim 3D object detector. In a certain degree, a mis-categorization attack can also be seen as the variation of a disappearing attack, since they both use the similar methods to manipulate the victim's prediction results to an existed objects.}

Compared with appearing attacks, we argue that a disappearing attack \xqf{or a mis-categorization attack are} less threatening in the real world because {they are both untargeted and single-shot} at the self-driving level.
\xqf{For both two attacks, }the attacker has to put a printed object on the road or near some objects in preparation, which means he/she cannot choose the victim ADS during the attack.
Moreover, the printed object can only take effect once because it might be destroyed or recognized by the people nearby after the first accident of each attack.
% On one hand, 
% to implement a disappearing attack, the attacker has to put the printed objects on the road or near some objects before the attack happens,
% which means the attack can not choose the victim ADS.
% On the other hand, after the first accident of disappearing attack, a printed object may be destroyed and the people nearby may realize that there is probably some problems with the printed object, so it is hard for the attacker to use the same printed object to cause the second accident.
In contrast, in an appearing attack the attacker can choose the victim to fire the laser and forge non-existent cars as he/she wishes. Meanwhile, it is hard for others to notice this attack because there is almost no evidence left in the accident scene.

\xqf{Although due to the attack goal, it is meaningless to deploy LOP to defend against disappearing attacks, it is still worthwhile to evaluate the performance of LOP under mis-categorization attacks. We evaluate the performance of 3D object detectors under mis-categorization attacks in Appendix \ref{appendix:miscategorization}, and prove that LOP is also robustness against such attacks.}

% \noindent\textbf{Threats of Backdoor Attacks.}
\xqf{At last, }Backdoor attack is another threatening attack class to DNN models, which injects one or multiple backdoors into the victim model by modifying the training data \cite{chen2017targeted,turner2019labelconsitent}, the parameters \cite{jacob2020backdoorCNN,adnan2020TBT} or the network structure \cite{ruixiang2020embarrass}. After the injection, the adversary can activate his/her specified model misbehaviors by feeding special inputs containing the related trigger pattern. However, to implement a backdoor attack on the victim ADS is unrealistic. For example, the attacker requires the permission of the victim's self-driving system, which only belongs to a few administrators or security operators.
% Besides, with such permission, the attacker is able to directly modify the outputs of any DNN models, or even any modules in the self-driving system.
% Besides, even with such permission, the attacker has no need to backdoor is able to modify any modules in the self-driving system, or even the outputs of DNN models directly.
% Therefore, we believe that it is hard for an attacker to acquire the permission, and,
% once getting the permission, the attacker does not need to implement such a backdoor attack because he/she can already manipulate the victim as his/her wish.

% If the input of target model doesn't activate any triggers, the target model will return the normal prediction as usual.
% Otherwise, the target model will return a specific prediction which is linked with the activated trigger by the attacker.

% In 2017, Chen et al. firstly apply backdoor attack in machine learning, and suggest a \louis{fixed-pattern} backdoor attack: the trigger in the target model will be activated by a fixed pattern in the input \cite{chen2017targeted}.
% Turner et al. suggest not to change the labels of backdoor samples \louis{added} into the target model's training set, and improve the invisibility of backdoor attack during the training stage of target model \cite{turner2019labelconsitent}.
% On the other hand, Li et al. and Pang et al. suggest dynamic-pattern backdoor attacks, where the trigger in the target model will be activated by different patterns for different inputs, and improve the invisibility of backdoor attack during the inference stage of target model \cite{li2019invisible,pang2020atale}.
% The studies above prove that backdoor attacks can manipulate the target model's output on specific tasks, without harming the model's performance on its main task or being noticed by others.


% he/she doesn't need to implement backdoor attack while he/she is able to manipulate the victim as his/her wish. 

\xqf{\noindent\textbf{Other Potential Defenses.}
Except those defense methods we mentioned in Section \ref{sec:Limitation}, the fusion strategy is also a choice to defend against appearing attacks. Different from most existing defenses, fusion strategy can also improve the performance of the object detectors by taking images as the auxiliary inputs. Furthermore, \cite{Hallyburton2021SecurityAO} has already proved that the Physical attack can not break most of the fusion model such as FCN, FPN and AVOD.}

\xqf{However, according to \cite{yulan2021deep}, the detection frequency of existing fusion models is usually lower than $15$ FPS, and we are afraid but current fusion models may not be suitable for real-time self-driving system due to the efficiency bottleneck. Besides, we argue that fusion models should be viewed as also one of the defense targets instead of the comparison groups to our proposed defense, since they are also by essence detectors. Due to the plug-in nature of LOP, we are further able to equip the fusion models with LOP to defend against appearing attacks. Furthermore, we evaluate the performance of one of the fusion models with our proposed defense under different appearing attacks in Appendix \ref{appendix:fusion}, and prove that LOP empirically improves the robustness of the fusion models.}

\noindent\textbf{Limitations and Future Directions.} 
% Although there may be potential adaptive attacks designed to break the LOP in the future, we argue that it is hard to implement in the real world. It is mainly because: 
% (i) Even the open-sourced ADS such as Apollo \cite{Apollo} keeps some small DNN models as black boxes. For example, there is a black-box DNN model used to locate the ADS in Apollo. The structure of this model is stored as an executable and linking file (*.so), and the parameter of this model is stored as an encrypted binary file (*.bin), which are difficult for attackers to decipher. Thus, it is also possible to protect the LOP by encrypting.
% (ii) The output of LOP is only a binary value to indicate the object is real or fake. Once the LOP is accessed as a black-box executable, it is generally hard for attacker to efficiently generate adversarial examples against our defense via optimization-based techniques.
% \morinop{(add discussion on adaptive attacks)}

\xqf{Although our proposed defense performs well in most cases in our experiments, there still exists some limitations of LOP to be solved:
(i) With the development of laser technology, the upper bound on the number of fake points generated by the attacker's equipment may keep increasing. In the future, the attacker may be capable to forge a car by copying all the points of a real car, which was almost impossible for LOP or other potential defenses to distinguish the difference.
(ii) By analyzing the false positives detected by LOP, we found that LOP performs not good enough on discriminating distant objects. Despite this, the existence of MOT module guarantees that erasing a real object in a few times will not harm too much on tracking its trajectory, and the influence of these distant objects on the route planning of ADS in a short time is limited. The further visualization and analysis of the main factor of these false positives are also shown in Appendix \ref{appendix:FP}.}


In this situation, it is almost impossible for a single LiDAR-based object detector and also the LOP to distinguish real and forged objects as their PCs are completely identical. Therefore, we believe that the fusion of multiple object detectors,
which combines multi-modal information from different sensor sources (e.g., cameras, LiDARs, radars) and different DNN models for a comprehensive prediction \cite{xiaozhi2017mv3d, gregory2019lasernet++, anas2021seqFusion},
is a promising way to alleviate the threats from the appearing attack, the disappearing attack or more unknown threats against object detectors. However, we should bear in mind that fusion is simply a mechanism which ensembles the capability of multiple DNN models and no more than such a mechanism. On one hand, to break the fused detector, the attacker needs to manipulate the outputs of all the component detectors, which means he/she has to modify the sampled data of multiple sensors towards the same attack goal without raising other modules' suspicion. On the other hand, to improve the robustness of each single component in the complex ADS is still meaningful and urging.  
For example, Cao et al. have already successfully broken a fused detector which combines image-based YOLO and Apollo's LiDAR-based object detector by disappearing attacks\cite{yulong2021invisible}.
% However, Cao et al. have already successfully broken a fused detector fusing YOLO and Apollo's LiDAR-based object detector \cite{yulong2021invisible},
% which proves that fusion is not the final solution to these latent attacks for ADS.
% Thus, we believe that our work also makes a little contribution to the security improvement of ADS.
Therefore, how to improve the robustness of a single object detector is crucial to the security of ADS, on which our current work focuses.

% Therefore, we believe that in order to eliminate the threat from appearing attack, other adversarial attacks or other attacks against object detectors, the most suitable way is to fuse multiple object detectors which take sampled data from different sensors, e.g. cameras, LiDARs and radars, as model's input \cite{xiaozhi2017mv3d, gregory2019lasernet++, anas2021seqFusion}.

==> tex/leftoff.tex <==
Formally,   Specifically, we propose to split the input space of each original training samples into equal-size small pillars, and annotate the  for our LOP based on the pillars. Specifically, we construct pairs of training samples for LOP solely with a standard training dataset for LiDAR-based object detectors (e.g., KITTI \cite{andreas2012kitti}). 

, i.e., the true spatial and semantic information of a real object present in input, 

In the past decade, deep learning has experienced great achievements in many domains such as finance \cite{Heaton2016DeepLF}, healthcare \cite{Esteva2017DermatologistlevelCO} and transportation \cite{edward2016doctorai,jiaxuan2019anAutomated}, 
bringing evolutionary changes to the industry landscape.
Among these, a

\louis{For more detailed analysis, please see Section \ref{sec:method:preparation}}

% Besides, the differences of defense effect between the 3D object detector with our LOP and the 3D object detector with SOR Besides, the differences of defense effect between our LOP and SOR are less than $5\%$ in most cases.


==> tex/relatedwork.tex <==
\section{Related Work}
\subsection{3D Object Detection}
[TBC]

\subsection{Appearing Attack}
[TBC]

\subsection{Certified Defense}
[TBC]
[Need to Discuss]
